RL-LABEL: A Deep Reinforcement Learning Approach Intended for AR Label Placement in Dynamic Scenarios

Labels are widely used in augmented reality (AR) to display digital information. Ensuring the readability of AR labels requires placing them occlusion-free while keeping visual linkings legible, especially when multiple labels exist in the scene. Although existing optimization-based methods, such as force-based methods, are effective in managing AR labels in static scenarios, they often struggle in dynamic scenarios with constantly moving objects. This is due to their focus on generating layouts optimal for the current moment, neglecting future moments and leading to sub-optimal or unstable layouts over time. In this work, we present RL-LABEL, a deep reinforcement learning-based method for managing the placement of AR labels in scenarios involving moving objects. RL-LABEL considers the current and predicted future states of objects and labels, such as positions and velocities, as well as the user's viewpoint, to make informed decisions about label placement. It balances the trade-offs between immediate and long-term objectives. Our experiments on two real-world datasets show that RL-LABEL effectively learns the decision-making process for long-term optimization, outperforming two baselines (i.e., no view management and a force-based method) by minimizing label occlusions, line intersections, and label movement distance. Additionally, a user study involving 18 participants indicates that RL-LABEL excels over the baselines in aiding users to identify, compare, and summarize data on AR labels within dynamic scenes.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> tex/_deprecated/1-intro_v1.tex <==
%% the only exception to this rule is the \firstsection command
\firstsection{Introduction}

\maketitle

Recent advances in low-cost consumer-level augmented reality (AR) devices, such as mobile phone or head mounted displays (HMDs), 
has been continuously gaining traction from the VIS research community~\cite{}.
These AR devices can blend the digital information with the physical environments in anywhere at any moment,
benefiting a wide range of applications in which the users need to consume information in-situ,
such as sports analytics~\cite{},  mechanical maintenance and repair~\cite{}, and medical surgery~\cite{}.
Fundamentally, AR platform can be seen as a ``superset'' of the desktop computer platform,
meeting human's information need in a border scenarios beyond the traditional in-door workspace~\cite{},

A widely-recognized promise from AR is to display extra digital information for real-world physical objects. 
In many AR applications~\cite{}, 
such digital information is commonly displayed as labels.
A label is a small virtual canvas placed in either the 3D world space or the 2D screen space,
connecting to the physical objects through a leader line.
A prerequisite before designing the visual representations of the information on the label is to decide the placement or layout of the labels.
Thus, extensive research~\cite{} has been proposed to automatically generating and managing
the layout of AR labels.
Most of the existing methods
formulate the layout problem as an optimization problem
and develop view management systems that generate 
layouts to maximize a set of objectives, 
such as avoiding overlaps between labels and objects~\cite{}, intersections between leader lines~\cite{},
and large distances between a label and its physical referents~\cite{}.
While these methods have been demonstrated their effectiveness for managing the layout of AR labels,
they mainly focus on static AR scenarios, in which the physical objects are placed in fixed positions.
However, in a real-world environment, the physical objects (such as sports players, pedestrians) are usually dynamic and change their positions frequently,
leading to a great demand of view management systems for AR labels in dynamic scenarios.

%% 
Managing the layout of AR labels for moving objects is challenging.
Compared to labels in static scenarios,
the labels in dynamic scenarios must update their positions to follow the moving objects continuously and stably,
while fulfilling the desired objectives (\emph{e.g.}, occlusion-free, line intersection-free).
% In other words, 
% the view management systems for dynamic scenarios need to control the movements
% of the labels rather than just their placements.
This requires the view management systems to generate label layouts
that should not only be optimal for the current moment 
but also can smoothly transfer to an optimal layout for the next moment.
Unfortunately, 
existing optimization-based methods can only 
generate optimal layouts for the current moment
but fail to take the next moment into account,
leading to sub-optimal or unstable layouts over time.
For example, \cmo{xxx}.
This is because the real-world environment is a partially observable environment,
in which the next position of a moving object and how it will move to the position
are unknown for the view management systems.

% make decisions for the labels' movements based on their current or historical states,
Inspired by other applications in partially observable environments (\emph{e.g.}, self-driving cars, robotics control),
we approach the view management of AR labels for moving objects from a new angle:
view management system is regarded as a sequential decision maker ($\uppi$)
that decides the movements of labels $\mathbf{a}_t$ 
at moment $t$ from the current state $\mathbf{s}_t$, \emph{i.e.}, $\uppi: \mathbf{s}^t \mapsto \mathbf{a}^t$.
% that can lead to maximal rewards in the long run, \emph{i.e.}, \cmo{xxx}.
We hereby introduce \cmo{SYSTEM}, 
a deep reinforcement learning-based method to seek an optimal decision maker that 
can lead to maximal rewards in the long run.
% a deep reinforcement learning-based method that approximates the optimal decision maker
\cmo{SYSTEM} xxxx

==> tex/_deprecated/2-realted_v1.tex <==
\newpage

\section{Related Work}

\begin{figure}[h]
  \centering
  \includegraphics[width=1\linewidth]{figures/fig_2Dvs3D labels.png}
  \caption{\cmo{Consider a scene with a blue 3D cube, which is projected to a
light-blue image in the image plane (black frame): (a) View management
in image space projects objects first and then places labels in 2D. (b)
View management in object space places labels in 3D and then projects
them to the image plane.}}
%   \Description{}
  \label{fig:2d_vs_3d}
\end{figure}


\para{Labeling in AR.}
Labels, a fundamental method to display extra information,
have been used for centuries to annotate objects in the context of illustrations~\cite{}.
Designers used to manually place labels in the illustrations to achieve a good readability
by avoiding overlapping between labels and objects, 
line intersections, 
and long distances between labels and their annotated objects, \emph{etc.}
In the early 80's, computer graphics researchers started to develop automated method,
or view management systems,
for placing labels.
Numerous research has been proposed in the past decades
to automatically place different labels (internal \emph{vs.} external)
in different environments ().
This work focuses on placing external labels in AR environments.

to study placing labels automatically in different conditions~\cite{} 
label styles (internal \emph{vs.} external)

The challenges of automatically placing labels come from 
the various labeling conditions and constraints
from, \emph{e.g.}, annotated objects (static \emph{vs.} dynamic),
placement spaces (2D \emph{vs.} 3D),
styles (internal \emph{vs.} external),
and environments (digital \emph{vs.} physical).
Even finding an optimal layout of labels for 2D illustrations has been shown to be a NP-hard problem~\cite{}.

Consequently, 


% When creating labels for illustrations, the most critical and challenging task is to place labels in proper positions so that they are not occluding important features and are still easy for the viewer to link between labels and illustration elements.

%% 2D, screen space
The view management systems~\cite{} for AR developed in the early 21st century
mainly placed and optimized the labels in the 2D screen space (so called 2D labels).
For example, Azuma and Furmanski~\cite{} employed a set of clustering strategies to the 2D labels.
As mentioned, optimal 2D label placement is an NP-hard problem. 
To approximate this problem, Azuma and Furmanski~\cite{} employed a set of clustering strategies to first identify local solutions and then combine them to a global solution.
An empirical study was conducted to evaluate the readability of the labels.
Grasset et al.~\cite{} proposed a image-based method that placing labels in unimportant regions by leveraging saliency detection.
To reduce the visual clutter when there is a large number of labels, 
they conducted a small-scale user study with 7 participants and found their participants generally preferred their technique over some other placement strategies.
Tatzgern et al.~\cite{} introduced an adaptive method to automatically cluster
labels based on the information density.


Label placement becomes more challenging when the viewing position and direction change over time.

However, 2D labels are suffered from ``floating labels'' problem~\cite{} -- when the user changes the viewpoint (which happens frequently in AR),
the labels will be re-layout and prone to unpredictable positions because the projected 3D points changes during camera movements.
To tackle this problem, 
researchers thus have developed view management systems for 3D AR labels that are placed in 3D object space.
Hedgehog labeling, a representative example of 3D labels presented by Tatzgern et al.~\cite{},
used 3D geometric constraints to generate label placements that fulfilled both the desired objectives (\emph{e.g.}, occlusion free) and stability over time when the viewpoint changes.
Their method was then compared with 2D labels by Madsen et al.~\cite{} in an emprical study.
Findings revealed that 3D labels with a limited update rate outperformed 2D labels and 3D labels updated continuously.
More recently, Koppel et al.~\cite{} contributed a systems for 3D AR labels 
that managed the label visibility and level-of-detail, considering both the labels in front of 
and out of the view. Gebhardt et al.~\cite{} utilized reinforcement learning to
control to visbility of an object's label based on the user's eye movement data.
Lin et al.~\cite{} studied the design space of both 2D and 3D AR labels for out-of-view objects.

While these AR labeling methods have been demonstrated their usefulness and effectiveness in different AR scenarios,
they all focused on static objects with fixed position in the scene.
However, in AR environments, objects are usually dynamic and moving from time to time (e.g., basketball players on the court, advertisements on moving vehicles, sushi on a belt conveyor).
The objects' movements are usually unknown beforehand,
posing extra challenges to place the labels.
\cmo{should expand a bit about the challenge}
We thus aim to
develop a view management system that observers the real-world environments
and adapts the 3D labels to the dynamic moving objects in real-time.


However, to the best of our knowledge, there is no previous research about how to best place labels in 3D space for dynamic (or moving) objects in AR.
This project fills the gap by applying reinforcement learning for real-time 3D dynamic label placement in AR, and comparing it to an  adaption from the state-of-the-art static labeling technique, as well as the naive placement strategy without any optimization.

\para{Adaptive User Interfaces in Augmented Reality.}
Labels are a kind of user interfaces (UIs) that display visual content in small canvases~\cite{}.
Different from UIs in traditional desktop environments,
UIs in AR are inherently context-sensitive~\cite{} and need to adapt to the users' environments
in real-time as many design decisions of the UIs cannot be made in advance, such as where and how they should be displayed.
Extensive research~\cite{} has been conducted to ease this problem by making the UIs adapt to the real-world environments in real-time.
A variety of works have leveraged the geometry information of the surroundings to determine the UI placements. Typically, AR contents can be placed on surfaces~\cite{}, aligned with edges~\cite{},
and interacted with 3D meshes~\cite{} detected and extracted from the physical environments.
This spatial information enables fundamental AR features such as providing physical referets for the virtual content and thus has been used
in most of the AR applications~\cite{}.

In addition to basic geometry information, most recent AR UIs leverage semantic information
of the scene to provide more engaging AR experience.
For instance, 
Tahara et al.~\cite{} employed a scene graph to define the spatial relationships between virtual and physical objects, automatically adjusting the virtual content when the user moved to other enviornments.
AdapTutAR~\cite{}, an AR task tutoring system, adjusted the teaching content adapatively based on
the user's characteristics.
SemanticAdapt~\cite{} used computer vision techniques to detect the category of real objects 
and associated them with AR content.
Lindlbauer et al.~\cite{} controlled the placement and level-of-detail of virtual content
considering both the indoor environment and the cognitive load of the user's performing task.
ScalAR~\cite{} enabled designers to author semantically adaptive AR experiences in VR.
However, all these works focused on scenarios where 
the UIs are adjusted infrequently,
such as re-positioning the AR UIs when the user moves from one room to the other.
Moreover, the physical objects are usually static with a fixed position.
We share a similar spirit with these works but target a different AR scenario,
wherein the objects are moving and the AR UIs need to be updated continuously.

\para{AR Labeling as a Partially Observable Decision Problem.}
Fundamentally, managing labels for moving objects in AR is a partially observable decision problem~\cite{}.
In a partially observable environment, the entire state is partially visible to external sensors.
For example,
the moving destination and route planned of a real object are only known by the object itself but agnostic for others.
This is an essential difference between managing labels for moving objects in AR and VR or 3D environments, 
in which the system state is fully visible to the system.
Typical applications of partially observable problems include self-driving car~\cite{}, robotics control~\cite{}, and card games~\cite{}.
Recently, deep reinforcement learning (RL) has demonstrated promising performance in facilitating these applications.
% solving partially observable decision problems.
Inspired by these applications, this work explores leveraging deep RL to manage the labels of dynamic moving objects in AR.
% Thus, the view management system has to observe and predict the movements of the objects and 
% forcing the view management system to predict and plan the label layout 
% and are agnostic for the view management system.

\para{Reinforcement Learning for Data Visualizations.}
In reinforcement learning, 
an agent observes an environment
and learns to take actions to maximize the cumulative rewards. 
Different from supervised and unsupervised learning 
in which the models learn from the historical data,
the models of RL learn
from the interactive experiences with the environments (\emph{e.g.}, playing a GO game).
The learned policies can be applied to control agents in the similar environments.
Thus, reinforcement learning has been widely used in dynamic scenarios
to solve problems that involve a huge solution space or require a long-run optimization.
RL is a promising technique for solving some specific visualization problems. However, to the best of our knowledge, there are only a few studies have explored applying RL methods to improve visualization~\cite{}.
% In the visualization community, however, 
% only a few studies have explored using RL methods
% to solve visualization problems~\cite{}.
For example, PlotThread~\cite{} utilized a RL-based method
to create user-preferred storyline layouts 
by formalizing the problem as performing
a sequence of layout modifications on a less satisfying layout,
wherein the layout is the environment and the modifications are the actions taken by the agent.
MobileVisFixer~\cite{} employed RL methods to learn policies to adapt visualizations
to different mobile devices by adjusting their parameters such as size, offset, and margin.
In MobileVisFixer, the environment is the the dimensions of the mobile devices.
Table2Chart~\cite{} used deep Q-learning to recommend chart templates based on the data tables.
In summary, most of the existing works of using RL for data visualizations focus on static 2D environments,
while our goal is to use RL-based methods to manage the layout of labels in dynamic 3D environments,
which is an underexplored direction and poses more challenges.


% \subsection{Dynamic Visualizations}

% https://www.microsoft.com/en-us/research/wp-content/uploads/2016/02/tvcg2008-trendvis.pdf

% http://vis.stanford.edu/files/2007-AnimatedTransitions-InfoVis.pdf

==> tex/_deprecated/2-related_v2.tex <==
\newpage

\section{Related Work \cmo{within one page}}

\begin{figure}[h]
  \centering
  \vspace{-10mm}
  \includegraphics[width=0.85\linewidth]{figures/fig_2dvs3d.png}
  \caption{\cmo{Consider a scene with a blue 3D cube, which is projected to a
light-blue image in the image plane (black frame): (a) View management
in image space projects objects first and then places labels in 2D. (b)
View management in object space places labels in 3D and then projects
them to the image plane.}}
%   \Description{}
  \label{fig:2d_vs_3d}
\end{figure}

\para{Labeling in AR.}
Labels are a fundamental means to display extra information, and
have been used for centuries to annotate objects in the context of illustrations~\cite{}.
Originally, designers placed labels manually in illustrations, aiming to achieve good readability of labels by avoiding overlapping labels and objects, line intersections, and long distances between labels and their annotated objects, \emph{etc.}
In the early 80's, computer graphics researchers started to develop automated methods, or view management systems, for placing labels.
%
Methods differ by the type of labels they support (internal~\cite{} \emph{vs.} external~\cite{}) and their intended environment (desktop~\cite{} \emph{vs.} AR~\cite{}).
%Different methods target labels with different styles (internal~\cite{} \emph{vs.} external~\cite{}) in different environments (desktop~\cite{} \emph{vs.} AR~\cite{}).
This work focuses on placing external labels in AR environments.

% Even finding an optimal layout of labels for 2D illustrations has been shown to be a NP-hard problem~\cite{}.

% When creating labels for illustrations, the most critical and challenging task is to place labels in proper positions so that they are not occluding important features and are still easy for the viewer to link between labels and illustration elements.

%% 2D, screen space
Early view management systems~\cite{} for AR environments mainly place labels in 2D screen space (\autoref{fig:2d_vs_3d}a).
These 2D labels only exist in the view plane and are not affected by any 3D transformations.
For example, Azuma and Furmanski~\cite{} presented a method that identifies clusters of labels in screen space and 
generates new positions for them.
% An empirical study revealed that their method can generate label layouts with good readability.
% employed a set of clustering strategies to the 2D labels.
% To approximate this problem, Azuma and Furmanski~\cite{} employed a set of clustering strategies to first identify local solutions and then combine them to a global solution.
Grasset et al.~\cite{} proposed an image-based method that places labels in unimportant regions by leveraging saliency detection.
% They conducted a small-scale user study with 7 participants and found their participants generally preferred their technique than some other placement techniques.
To reduce visual clutter when there is a large number of labels, 
Tatzgern et al.~\cite{} introduced an adaptive method to automatically cluster labels based on information density.
However, 2D labels suffer from the ``floating labels'' problem~\cite{} -- when the user changes the viewpoint (which happens frequently in AR), the labels will be re-positioned, which can lead to unpredictable label positions because the projected 3D points change during camera movements.

Compared to 2D labels, 3D labels placed in 3D object space (\autoref{fig:2d_vs_3d}b)
are more stable even when the user changes the viewpoint in AR.
% To tackle this problem, 
% researchers have developed view management systems for 3D AR labels that are placed in 3D object space .
Tatzgern et al.~\cite{} proposed Hedgehog labeling, a representative example of 3D labels. 
They use 3D geometric constraints to generate label placements that fulfill the desired objectives (\emph{e.g.}, being occlusion free) and are stable over time, even when the viewpoint changes.
Madsen et al.~\cite{} later compared this method to 2D labels in an emprical study.
Findings revealed that 3D labels with a limited update rate outperformed 2D labels and 3D labels that were updated continuously.
More recently, Koppel et al.~\cite{} contributed a systems for 3D AR labels that manages label visibility and level-of-detail, considering both the labels in front of and out of the view. 
Gebhardt et al.~\cite{} utilized reinforcement learning to
control to visbility of an object's label based on the user's eye movement data.
Lin et al.~\cite{} studied the design space of both 2D and 3D AR labels for out-of-view objects.

While the above methods have demonstrated their usefulness and effectiveness in different AR scenarios,
they all focus on static objects with fixed positions in the scene.
However, in AR environments, objects are usually dynamic and moving from time to time 
(\emph{e.g.}, basketball players on the court, advertisements on moving vehicles, sushi on a conveyor belt).
The objects' movements are usually unknown beforehand,
posing extra challenges to place the labels.
\cmo{should expand a bit about the challenge}
We thus aim to
develop a view management system that observes the real-world environment and adapts the 3D labels to the dynamic moving objects in real-time.

% However, to the best of our knowledge, there is no previous research about how to best place labels in 3D space for dynamic (or moving) objects in AR.
% This project fills the gap by applying reinforcement learning for real-time 3D dynamic label placement in AR, and comparing it to an  adaption from the state-of-the-art static labeling technique, as well as the naive placement strategy without any optimization.

\para{Adaptive User Interfaces in Augmented Reality.}
A label is a type of user interface (UI) that displays visual content in a small canvas~\cite{}.
Different from UIs in traditional desktop environments, UIs in AR are inherently context-sensitive~\cite{} and need to adapt to the user's environment in real-time. Many design decisions of UIs in AR cannot be made in advance, such as where and how they should be displayed.
Extensive research~\cite{} has been conducted to ease this problem by making UIs adapt to real-world environments in real-time.
A variety of works have leveraged geometry information of the surroundings to determine UI placement. Typically, AR content can be placed on surfaces~\cite{}, be aligned with edges~\cite{},
and interacted with 3D meshes~\cite{} that have been detected and extracted from the physical environment.
This spatial information enables fundamental AR features such as providing physical referents for the virtual content and thus has been used in many AR applications~\cite{}.

In addition to basic geometry information, some recent AR UIs leverage semantic information of the scene to provide a more engaging AR experience.
For instance, Tahara et al.~\cite{} employ a scene graph to define the spatial relationships between virtual and physical objects, automatically adjusting the virtual content when the user moves to other environments.
AdapTutAR~\cite{}, an AR task tutoring system, adjusts the teaching content adapatively based on the user's characteristics.
SemanticAdapt~\cite{} uses computer vision techniques to detect the category of real objects and associates them with AR content.
Lindlbauer et al.~\cite{} controls the placement and level-of-detail of virtual content by considering both the indoor environment and the cognitive load of the user's performing task.
ScalAR~\cite{} enables designers to author semantically adaptive AR experiences in VR.
However, all these works focus on scenarios where the UIs are adjusted infrequently, such as re-positioning the AR UIs when the user moves from one room to the other.
Moreover, the physical objects are usually static with a fixed position.
We share a similar spirit with these works but target a different AR scenario, wherein the objects are moving and the AR UIs need to be updated continuously.

\para{AR Labeling as a Partially Observable Decision Problem.}
Fundamentally, managing labels for moving objects in AR is a partially observable decision problem~\cite{}.
In a partially observable environment, the entire state is partially visible to external sensors.
For example,
the moving destination and route planned of a real object are only known by the object itself but unknown to others.
This is an essential difference between managing labels for moving objects in AR compared to desktop 3D environments, 
where the system state is fully visible to the system.
Typical applications of partially observable problems include self-driving cars~\cite{}, robotics control~\cite{}, and card games~\cite{}.
Recently, deep reinforcement learning (RL) has demonstrated promising performance in facilitating these applications.
% solving partially observable decision problems.
Inspired by these applications, this work explores leveraging deep RL to manage the labels of dynamically moving objects in AR.
% Thus, the view management system has to observe and predict the movements of the objects and 
% forcing the view management system to predict and plan the label layout 
% and are agnostic for the view management system.

\para{Reinforcement Learning for Data Visualizations.}
In reinforcement learning, a model observes an environment and learns to take actions to maximize some cumulative rewards. 
Different from supervised and unsupervised learning 
in which the models learn from the historical data,
the models of RL learn
from the interactive experience with the environment (\emph{e.g.}, playing a GO game).
The learned policies can be applied to control agents in similar environments.
Thus, reinforcement learning has been widely used in dynamic scenarios to solve problems that involve a huge solution space or require a long-run optimization.
% RL is a promising technique for solving some specific visualization problems. 
% However, to the best of our knowledge, there are only a few studies have explored applying RL methods to improve visualization~\cite{}.
% In the visualization community, however, 
% only a few studies have explored using RL methods
% to solve visualization problems~\cite{}.
In the visualization community, to the best of our knowledge,
only a few studies have explored using RL methods
to solve visualization problems~\cite{}.
For example, PlotThread~\cite{} utilizes an RL-based method
to create user-preferred storyline layouts 
by formalizing the problem as performing
a sequence of layout modifications on a less satisfying layout,
wherein the layout is the environment and the modifications are the actions taken by the agent.
MobileVisFixer~\cite{} employs RL methods to learn policies to adapt visualizations
to different mobile devices by adjusting their parameters such as size, offset, and margin.
In MobileVisFixer, the environment corresponds to the dimensions of the mobile device.
Table2Chart~\cite{} uses deep Q-learning to recommend chart templates based on given data tables.
In summary, most of the existing works using RL for data visualization focus on static 2D environments,
while our goal is to use RL-based methods to manage the layout of labels in dynamic 3D environments,
which is an underexplored direction and poses more challenges.


% \subsection{Dynamic Visualizations}

% https://www.microsoft.com/en-us/research/wp-content/uploads/2016/02/tvcg2008-trendvis.pdf

% http://vis.stanford.edu/files/2007-AnimatedTransitions-InfoVis.pdf

==> tex/_deprecated/3-problem_v1.tex <==

\section{Problem Formulation}

This work considers scenarios where the viewer stays at a fixed position to watch multiple objects moving in the view,
such as watching sports in a stadium 
and monitoring an environment using surveillance cameras.
We constraint that each object is annotated by a single label
and leave the multiple-label scenarios for future research.
% At moment $t$,
Three components are involved in the view management process:
\begin{itemize}%[leftmargin=*]
    \item \textbf{Object:} 
    % A scene usually contains a set of objects $\{\textbf{o}^i\}^n_{i=1}$
    % An object set $O$ contains $n$ objects $\{\textbf{o}^i\}^n_{i=1}$, 
    % each of which is 
    An object $\mathbf{o}^i$ can be approximated as a cube shape rigid body 
    in the 3D \emph{world} space $\mathbb{R}^3_{wld}$.
    The object $\mathbf{o}^i$ attempts to move to a goal position $\mathbf{p}_g^i$ following a planned route and a preferred velocity.
    While its position $\mathbf{p}^{i,t} = (x^{i,t}, y^{i,t}, z^{i,t})$
    %, normal $\mathbf{n}^{i,t}=(n_x^{i,t}, n_y^{i,t}, n_z^{i,t})$
    and velocity $\mathbf{v}^{i,t} = (v_x^{i,t}, v_y^{i,t}, v_z^{i,t})$ at moment $t$ is observable,
    its goal position, 
    planned route, 
    and preferred velocity
    are unobservable
    for external observers, \emph{e.g.}, the view management system.
    Thus, 
    % at the moment $t$,
    the observable state of the object can be represented as $\mathbf{s}^{i,t}_{\mathbf{o}} = \{\mathbf{p}^{i, t}, \mathbf{v}^{i, t}\}$.
    The observable state of all the objects 
    % in the scene 
    $\mathbf{s}_{\mathbf{o}}^t$
    is thus $\{\mathbf{s}^{i,t}_\mathbf{o} \}^n_{i=1}$,
    where $n$ is the number of objects.
    
    \vspace{0.5mm}    
    \item \textbf{Label:} 
    % A label set $L$ consists of $n$ 3D labels $\{\mathbf{l_i}\}^n_{i=1}$, each of which annotates an object $\mathbf{o}$.
    A label $\mathbf{l}^j$ is a rectangle shape canvas placed at position $\mathbf{p}^j$ in the 3D \emph{world} space $\mathbb{R}^3_{wld}$, 
    linking to its target object $\mathbf{o}^j$ through a leader line.
    In practice, the label $\mathbf{l}^j$ usually keeps its normal $\mathbf{n}^{j,t} = (n_x^{j,t}, n_y^{j,t}, n_z^{j,t})$
    pointing 
    to the camera to maximize its readability.
    Thus, the observable state of the label $\mathbf{l}^j$ can be defined as
    $\mathbf{s}^{j,t}_\mathbf{l} = \{\mathbf{p}^{j,t}, \mathbf{v}^{j,t}, \mathbf{n}^{j, t}, \mathbf{s}^{j,t}_{\mathbf{o}}\}$,
    where 
    % $\mathbf{s}_{\mathbf{o}}^{j,t}$ is the observable state of its annotated object,
    $\mathbf{p}^{j,t}$, $\mathbf{v}^{j,t}$, $\mathbf{n}^{j, t}$, and $\mathbf{s}^{j,t}_{\mathbf{o}}$ 
    are its position, velocity, normal vector, 
    and the state of its target object $\mathbf{o}^j$, respectively.
    Similarly, 
    the state of all labels 
    $\mathbf{s}_{\mathbf{l}}^t$
    is represented by $\{\mathbf{s}^{j,t}_\mathbf{l} \}^m_{j=1}$, 
    where $m$ is the number of labels.
    In this work, $m$ equals $n$. 

    \vspace{0.5mm}
    \item \textbf{Viewpoint:} 
    A viewpoint specifies how the observer watches the objects and labels,
    which is 
    % The viewpoint is 
    determined by the camera $\mathbf{c}$.
    % Since that %in our scenario 
    % the observer stays at a fixed position 
    % and objects moves in the view,
    % we can assume that the camera parameters, 
    % including its position, projection types, and field of view (FOV),
    % are unchanged over time for simplification.
    Thus, the state of the viewpoint $\mathbf{s}^t_\mathbf{c}$ can be represented as the projection matrix $\mathbf{M}^t_{cam}$.
    % $\mathbf{s}^t_\mathbf{c} = \mathbf{M}^t_{cam}$, where $\mathbf{M}^t_{cam}$ is the projection matrix.
    % \cmo{Note that this simplification won't impoverish the generalizability of our approach as the translations of the camera can be converted to the relative movements of the objects.}

\end{itemize}

For a label $\mathbf{l}^{j}$,
a view management system can be regarded as a mapping function
$\uppi(\mathbf{s}_{\mathbf{l}}^{j, t}, 
% \mathbf{s}_{\mathbf{o}}^{j,t}, 
\mathbf{\Tilde{s}}_\mathbf{ol}^{j, t}, \mathbf{s}^t_\mathbf{c}) \mapsto \mathbf{a}^{j, t}$ %% \mapsto \mathbf{a}^{j,t}$,
that inputs 
the label's own state $\mathbf{s}_{\mathbf{l}}^{j, t}$, 
% the state of its target object $\mathbf{s}_{\mathbf{o}}^{j,t}$,
the states of all other objects and labels $\mathbf{\Tilde{s}}_{\mathbf{ol}}^{j, t} = \{\mathbf{s}_{\mathbf{o}}^t \setminus \{\mathbf{s}^{j,t}_\mathbf{o}\}, \mathbf{s}_{\mathbf{l}}^t \setminus \{\mathbf{s}^{j,t}_\mathbf{l}\} \}$,
and the viewpoint's state $\mathbf{s}^t_\mathbf{c}$,
and outputs an action $\mathbf{a}^{j, t}$ to update the label's position. % and velocity
This mapping process is repeated for each label at each timestamp.

% where 
% $\mathbf{\Tilde{s}}_{\mathbf{l}}^{j, t} = \{\mathbf{s}_{\mathbf{o}}^t, \mathbf{s}_{\mathbf{l}}^t \setminus \{\mathbf{s}^{j,t}_\mathbf{l}\} \}$ 
% denotes the state of all objects and other labels except the label $\mathbf{s}_{\mathbf{l}}^{j, t}$,
% the output $\mathbf{a}^{j, t}$ is an action that updates the position and velocity of the label $\mathbf{s}_{\mathbf{l}}^{j, t}$.
% Intuitively, for each label, the view management system $\uppi$ updates its position and velocity based on its own state, the states of all objects and other labels, and the camera's state.
% Let $\mathbf{s}^t = \{\mathbf{s}_{\mathbf{o}}^t, \mathbf{s}_{\mathbf{l}}^t, \mathbf{s}_\mathbf{c}\}$.
% The view management system can be regarded as a mapping $\uppi: \mathbf{s}^t \mapsto \mathbf{a}^t$
% that outputs an action .
% \cmo{should give an example of action?}

Typically, a view management system should output actions to optimize the objectives.
% to avoid 
% 1) occlusions between labels and objects, 
% 2) intersections between leader lines, 
% 3) long distance between a label and its annotated object,
% and 4) abrupt moves of the labels~\cite{}.
We simplify the input of the view management system as 
$\mathbf{s}^{j, t} = \{\mathbf{s}_{\mathbf{l}}^{j, t}, \mathbf{\Tilde{s}}_\mathbf{ol}^{j, t}, \mathbf{s}^t_\mathbf{c}\}$.
We then can define a reward function $r(\mathbf{s}^{j, t}, \mathbf{a}^{j,t})$ to evaluate how good the action $\mathbf{a}^{j,t}$ achieves the objectives given the input $\mathbf{s}^{j, t}$.
A good view management system for dynamic scenarios should maximizes the reward in a long-run:

\begin{equation}\label{eq:pi}
    \arg \max_{\uppi} \{r(\mathbf{s}^{j,t}, \mathbf{a}^{j,t}) + \gamma V^*(\delta(\mathbf{s}^{j,t}, \mathbf{a}^{j,t})) | \uppi(\mathbf{s}^{j, t}) \mapsto \mathbf{a}^{j,t}\}
\end{equation}

% \begin{equation}\label{eq:v}
%     V(\mathbf{s}^{t+1}) = P(\mathbf{s}^{t+1} | \mathbf{s}^t, \mathbf{a}^t) \sum_{t' = t + 1}^{T} \gamma^{t'} R(\mathbf{s}^{t'}, \uppi(\mathbf{s}_{\mathbf{l}}^{j, t'}, \mathbf{\Tilde{s}}_{\mathbf{l}}^{j, t'}, \mathbf{s}^{t'}_\mathbf{c}))
% \end{equation}

\noindent
, where $\gamma$ is a discount factor,
$\delta(\mathbf{s}^{j,t}, \mathbf{a}^{j,t})$ represents the next state after applying action $\mathbf{a}^{j,t}$ under state $\mathbf{s}^{j,t}$,
$V^*$ is the optimal value function that estimate the optimal cumulative rewards from the input state to the future.
Simply put, 
\autoref{eq:pi} describes that
the optimal view management system $\uppi^*$ 
should generate actions to maximize not only the reward $r(\mathbf{s}^{j,t}, \mathbf{a}^{j,t})$ for the current state
but also the future cumulative rewards $\gamma V^*(\delta(\mathbf{s}^{j,t}, \mathbf{a}^{j,t}))$.

In this work,
we aim to solve Eq.~\ref{eq:pi} using deep RL methods.
Specifically, we train a neural network to approximate an optimal mapping function $\uppi$.
To assist in training the mapping function $\uppi$,
we also train a neural network to approximate the optimal value function $V^*$.

\para{The difference between RL- and optimization-based methods.}
Most of the existing view management systems for static objects use optimization-based methods to optimize the reward for the current state,
which is equivalent to solving the first part of Eq.\ref{eq:pi}, \emph{i.e.}, $\arg \max_{\uppi} \{r(\mathbf{s}^{j,t}, \mathbf{a}^{j,t}) \}$.
This is reasonable for objects that are static. 
However, for a dynamic scenario, 
optimization-based methods fall short to 
predict the movement of the objects
and cannot estimate the future impact of an action,
leading to sub-optimal results.
RL-based methods, on the other hand, have the potential to overcome this issue.

\para{The challenges of placing labels in AR \emph{vs}. similar dynamic scenarios.}
Compared to other similar dynamic 3D scenarios, such as VR or 3D games,
AR environments pose an unique challenge for placing labels of moving objects
in that the next state $\delta(\mathbf{s}^{j,t}, \mathbf{a}^{j,t})$ after applying action $\mathbf{a}^{j,t}$ 
is unknown,
% the transition probability function $P(\mathbf{s}^{t+1} | \mathbf{s}^t, \mathbf{a}^t)$
since how the objects will move in the next moment $t+1$ is agnostic for the view management system.
Hence, the output of the optimal value function $V^*$ is also unknown as it relies on the next state as input. 

\para{Centralized training and decentralized execution.}
\cmo{maybe too much to discuss here. Update: I actually forget what I want to say here}

==> tex/_deprecated/3-problem_v2.tex <==

\section{Problem Formulation}

This work considers scenarios where the viewer stays at a fixed position to watch multiple objects moving in the view,
such as watching sports in a stadium 
and monitoring an environment using surveillance cameras.
We constrain that each object is annotated by a single label
and leave multiple-label scenarios for future research.


\begin{figure}[h]
  \centering
  \includegraphics[width=1\linewidth]{figures/fig_problem.pdf}
  \caption{We consider scenarios where a stationary viewer observes multiple moving objects, each with a corresponding label. \cmo{to update}}
%   \Description{}
  \label{fig:problem}
\end{figure}


% At moment $t$,
\noindent
The view management process involves three components (\autoref{fig:problem}):
\begin{itemize}%[leftmargin=*]
    \vspace{1mm}
    \item \textbf{Object:} 
    An object $\mathbf{o}^i$ can be approximated as a cube shape rigid body 
    in the 3D \emph{world} space $\mathbb{R}^3_{wld}$.
    The object $\mathbf{o}^i$ attempts to move to 
    a goal position following a planned route and a preferred velocity.
    For a view management system,
    the observable state of the object     
    can be represented as 
    $\mathbf{o}^{i,t} = \{\mathbf{p}^{i, t}_\mathbf{o}, \mathbf{v}^{i, t}_\mathbf{o}, \mathbf{n}^{i,t}_\mathbf{o}\}$, 
    where $\mathbf{p}^{i,t}_\mathbf{o} = (x^{i,t}, y^{i,t}, z^{i,t})$,
    $\mathbf{v}^{i,t}_\mathbf{o} = (v_x^{i,t}, v_y^{i,t}, v_z^{i,t})$,
    and $\mathbf{n}^{i,t}_\mathbf{o} = (n_x^{j,t}, n_y^{j,t}, n_z^{j,t})$
    are its position, velocity, and normal at moment $t$, respectively.
    The observable state of all the objects 
    is thus $\mathbf{o}^{t} = \{\mathbf{o}^{i,t} \}^n_{i=1}$,
    where $n$ is the number of objects.
    
    \vspace{1mm}    
    \item \textbf{Label:} 
    A label $\mathbf{l}^i$ is a rectangle shape canvas in the 3D \emph{world} space $\mathbb{R}^3_{wld}$, 
    linking to its target object $\mathbf{o}^i$ through a leader line.
    The observable state of the label at the moment $t$
    can be defined as
    $\mathbf{l}^{i,t} = \{\mathbf{p}^{i,t}_\mathbf{l}, \mathbf{v}^{i,t}_\mathbf{l}, \mathbf{n}^{i, t}_\mathbf{l}, \mathbf{p}^{i,t}_{\mathbf{o}} \}$,
    where $\mathbf{p}^{i,t}_\mathbf{l}$, $\mathbf{v}^{i,t}_\mathbf{l}$, and $\mathbf{n}^{i,t}_\mathbf{l}$
    are its position, velocity, and normal, respectively; $\mathbf{p}^{i,t}_{\mathbf{o}}$ represents the other endpoint of the leader line.
    In practice, 
    the label usually keeps its normal $\mathbf{n}^{i,t}_\mathbf{l}$
    pointing to the camera to maximize its readability.
    Similarly, 
    the state of all labels 
    is represented by $\mathbf{l}^t = \{\mathbf{l}^{i,t} \}^n_{i=1}$, 
    where $n$ is the number of labels, which equals the number of objects.

    \vspace{1mm}
    \item \textbf{Viewpoint:} 
    A viewpoint is determined by the camera $\mathbf{c}$ and specifies the observer's position in relation to the objects and labels being watched. 
    Thus, at the moment $t$, the state $s$ of the viewpoint $\mathbf{c}^t$ can be represented as the projection matrix $\mathbf{M}^t_{cam}$.
    % \cmo{Note that this simplification won't impoverish the generalizability of our approach as the translations of the camera can be converted to the relative movements of the objects.}

\end{itemize}

For a label $\mathbf{l}^{i}$,
a view management system needs to generate 
an action $\mathbf{a}^{i, t}$ to update its position
based on its current state $\mathbf{l}^{i, t}$,
the states of its target object $\mathbf{o}^{i,t}$,
other labels $\mathbf{l}^t \setminus \{\mathbf{l}^{i,t}\}$,
other objects $\mathbf{o}^t \setminus \{\mathbf{o}^{i,t}\}$,
and the viewpoint $\mathbf{c}^t$.
We simplify the input of the system as 
$\mathbf{s}^{i, t} = \{
    \mathbf{l}^{i, t},~
    \mathbf{o}^{i,t},~
    \mathbf{l}^t \setminus \{\mathbf{l}^{i,t}\},~
    \mathbf{o}^t \setminus \{\mathbf{o}^{i,t}\},~
    \mathbf{c}^t
\}$.
Then, this process can be regarded as a mapping function:

\begin{equation}
\uppi(
\mathbf{s}^{i, t}
) \mapsto \mathbf{a}^{i, t} 
\end{equation}
This mapping process is applied on each label at each timestamp.


Typically, a view management system should output actions to optimize the objectives.
% to avoid 
% 1) occlusions between labels and objects, 
% 2) intersections between leader lines, 
% 3) long distance between a label and its annotated object,
% and 4) abrupt moves of the labels~\cite{}.
We can define a reward function $r(\mathbf{s}^{i, t}, \mathbf{a}^{i,t})$ to evaluate how good the action $\mathbf{a}^{i,t}$ achieves the objectives given the input $\mathbf{s}^{i, t}$.
A good view management system for dynamic scenarios should maximize the reward in a long run:

\begin{equation}\label{eq:pi}
    \arg \max_{\uppi} \{r(\mathbf{s}^{i,t}, \mathbf{a}^{i,t}) + \gamma V^*(\mathbf{s}^{i,t}, \mathbf{a}^{i,t}) | \uppi(\mathbf{s}^{i, t}) \mapsto \mathbf{a}^{i,t}\}
\end{equation}

\noindent
where $\gamma$ is a discount factor,
% $\delta(\mathbf{s}^{j,t}, \mathbf{a}^{j,t})$ represents the next state after applying action $\mathbf{a}^{j,t}$ under state $\mathbf{s}^{j,t}$,
$V^*$ is the optimal value function that estimates the optimal cumulative rewards to the future after performing action $\mathbf{a}^{i,t}$ under state $\mathbf{s}^{i,t}$.
Simply put, 
\autoref{eq:pi} describes that
the optimal view management system $\uppi^*$ 
should generate actions to maximize not only the reward $r(\mathbf{s}^{i,t}, \mathbf{a}^{i,t})$ for the current state
but also the future cumulative rewards $\gamma V^*(\mathbf{s}^{i,t}, \mathbf{a}^{i,t})$.

In this work, we aim to solve Eq.~\ref{eq:pi} using deep RL.
Specifically, we train a neural network to approximate an optimal mapping function $\uppi$.
To assist in training the mapping function $\uppi$,
we also train a neural network to approximate the optimal value function $V^*$.

\para{The difference between RL- and optimization-based methods.}
Most of the existing view management systems for static objects formulate the view management problem as an optimization problem
that aims to optimize the reward for the current state,
% use optimization-based methods to optimize the reward for the current state,
which can be represented by the first part of Eq.~\ref{eq:pi} 
(i.e., $\arg \max_{\uppi} \{r(\mathbf{s}^{i,t}, \mathbf{a}^{i,t}) \}$).
This approach is reasonable for static scenarios but falls short for dynamic ones,
because optimization-based methods cannot predict the movement of objects or estimate the future impact of an action, 
which thus leads to sub-optimal results. 
In contrast, RL-based methods have the potential to overcome these issues.

\para{The challenges of placing labels in AR vs. other 3D dynamic scenarios.}
Placing labels on moving objects in AR environments presents a unique challenge compared to other similar 3D dynamic scenarios, such as VR or 3D games. 
In 3D games, the system has full control of the objects and can \emph{plan} the best moving trajectories of the labels over time.
In contrast, in AR environments, the system can only observe the current state of the objects and is uncertain about their future states, 
such as their velocities. 
Therefore, the system must have the capability to predict future states to place the labels properly. 


% the optimal value function $V^*$ 
% is also unknown as it relies on the next state as input. 

% the next state $\delta(\mathbf{s}^{j,t}, \mathbf{a}^{j,t})$ after applying action $\mathbf{a}^{j,t}$ 
% is unknown,
% since how the objects will move in the next moment $t+1$ is agnostic for the view management system.

\para{Centralized training and decentralized execution.}
\cmo{maybe too much to discuss here. Update: I actually forget what I want to say here}
\cmo{update2: oh I remember. I want to say our method can run on each label in parallel (so called decentralized execution). The benefit of doing this is easy to scale up, adapt to dynamic environments, and save computational power. I think this part can be move to the next section. Let me think about it.}
